InfoBridge: Mutual Information estimation via Bridge Matching

Diffusion bridge models have recently become a powerful tool in the field of generative modeling. In this work, we leverage their power to address another important problem in machine learning and information theory, the estimation of the mutual information (MI) between two random variables. Neatly framing MI estimation as a domain transfer problem, we construct an unbiased estimator for data posing difficulties for conventional MI estimators. We showcase the performance of our estimator on three standard MI estimation benchmarks, i.e., low-dimensional, image-based and high MI, and on real-world data, i.e., protein language model embeddings.

==> gnuplot-lua-tikz-common.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%     Common style file for TeX, LaTeX and ConTeXt
%%  
%%  It is associated with the 'gnuplot.lua' script, and usually generated
%%  automatically. So take care whenever you make any changes!
%%

% check for the correct TikZ version
\def\gpchecktikzversion#1.#2\relax{%
\ifnum#1<2%
  \errmessage{PGF/TikZ version >= 2.0 is required!}%
\fi}
\expandafter\gpchecktikzversion\pgfversion\relax

\def\gnuplot@output@ps{ps} % required for comparison in \gprawimage

\expandafter\def\csname gnuplot@select@driver@pgfsys-dvi.def\endcsname     {ps}
\expandafter\def\csname gnuplot@select@driver@pgfsys-dvipdfm.def\endcsname {pdf}
\expandafter\def\csname gnuplot@select@driver@pgfsys-dvipdfmx.def\endcsname{pdf}
\expandafter\def\csname gnuplot@select@driver@pgfsys-dvips.def\endcsname   {ps}
\expandafter\def\csname gnuplot@select@driver@pgfsys-pdftex.def\endcsname  {pdf}
\expandafter\def\csname gnuplot@select@driver@pgfsys-luatex.def\endcsname  {pdf}
\expandafter\def\csname gnuplot@select@driver@pgfsys-tex4ht.def\endcsname  {html}
\expandafter\def\csname gnuplot@select@driver@pgfsys-textures.def\endcsname{ps}
\expandafter\def\csname gnuplot@select@driver@pgfsys-vtex.def\endcsname    {ps}
\expandafter\def\csname gnuplot@select@driver@pgfsys-xetex.def\endcsname   {pdf}

\ifcsname gnuplot@select@driver@\pgfsysdriver\endcsname
  \edef\gnuplot@output@mode{\csname gnuplot@select@driver@\pgfsysdriver\endcsname}
\else
  \errmessage{The driver \pgfsysdriver\space is not supported by gnuplot-lua-tikz}%
\fi

\ifcsname PackageWarning\endcsname
  \let\gnuplot@packagewarning\PackageWarning
\else
  \def\gnuplot@packagewarning#1#2{\immediate\write-1{Package #1 Warning: #2}}
\fi

% uncomment the following lines to make font values "appendable"
% and if you are really sure about that ;-)
% \pgfkeyslet{/tikz/font/.@cmd}{\undefined}
% \tikzset{font/.initial={}}
% \def\tikz@textfont{\pgfkeysvalueof{/tikz/font}}

%
% image related stuff
%
\def\gp@rawimage@pdf#1#2#3#4#5#6{%
  \def\gp@tempa{cmyk}%
  \def\gp@tempb{#1}%
  \ifx\gp@tempa\gp@tempb%
    \def\gp@temp{/CMYK}%
  \else%
    \def\gp@temp{/RGB}%
  \fi%
  \pgf@sys@bp{#4}\pgfsysprotocol@literalbuffered{0 0}\pgf@sys@bp{#5}%
  \pgfsysprotocol@literalbuffered{0 0 cm}%
  \pgfsysprotocol@literalbuffered{BI /W #2 /H #3 /CS \gp@temp}%
  \pgfsysprotocol@literalbuffered{/BPC 8 /F /AHx ID}%
  \pgfsysprotocol@literal{#6 > EI}%
}
\def\gp@rawimage@ps#1#2#3#4#5#6{%
  \def\gp@tempa{cmyk}%
  \def\gp@tempb{#1}%
  \ifx\gp@tempa\gp@tempb%
    \def\gp@temp{4}%
  \else%
    \def\gp@temp{3}%
  \fi%
  \pgfsysprotocol@literalbuffered{0 0 translate}%
  \pgf@sys@bp{#4}\pgf@sys@bp{#5}\pgfsysprotocol@literalbuffered{scale}%
  \pgfsysprotocol@literalbuffered{#2 #3 8 [#2 0 0 -#3 0 #3]}%
  \pgfsysprotocol@literalbuffered{currentfile /ASCIIHexDecode filter}%
  \pgfsysprotocol@literalbuffered{false \gp@temp\space colorimage}%
  \pgfsysprotocol@literal{#6 >}%
}
\def\gp@rawimage@html#1#2#3#4#5#6{%
  \gnuplot@packagewarning{gnuplot-lua-tikz}{%
    \noexpand\gp@rawimage is not implemented for \gnuplot@output@mode\space output.%
  }%
}

% Select \gp@rawimage depending on the output mode
\expandafter\let\expandafter\gp@rawimage\csname gp@rawimage@\gnuplot@output@mode\endcsname

\def\gploadimage#1#2#3#4#5{%
  \pgftext[left,bottom,x=#1cm,y=#2cm] {\pgfimage[interpolate=false,width=#3cm,height=#4cm]{#5}};%
}

\def\gp@set@size#1{%
  \def\gp@image@size{#1}%
}

\def\gp@rawimage@#1#2#3#4#5#6#7#8{%
  \tikz@scan@one@point\gp@set@size(#6,#7)\relax%
  \tikz@scan@one@point\pgftransformshift(#2,#3)\relax%
  \pgftext{%
    \pgfsys@beginpurepicture%
    \gp@image@size% fill \pgf@x and \pgf@y
    \gp@rawimage{#1}{#4}{#5}{\pgf@x}{\pgf@y}{#8}%
    \pgfsys@endpurepicture%
  }%
}

%% \gprawimage{color model}{xcoord}{ycoord}{# of xpixel}{# of ypixel}{xsize}{ysize}{rgb/cmyk hex data RRGGBB/CCMMYYKK ...}{file name}
%% color model is 'cmyk' or 'rgb' (default)
\def\gprawimage#1#2#3#4#5#6#7#8#9{%
  \ifx&#9&%
    \gp@rawimage@{#1}{#2}{#3}{#4}{#5}{#6}{#7}{#8}%
  \else
    \ifx\gnuplot@output@mode\gnuplot@output@ps
      \gp@rawimage@{#1}{#2}{#3}{#4}{#5}{#6}{#7}{#8}%
    \else
      \gploadimage{#2}{#3}{#6}{#7}{#9}%
    \fi
  \fi
}

%
% gnuplottex compatibility
% (see http://www.ctan.org/tex-archive/help/Catalogue/entries/gnuplottex.html)
%

\def\gnuplottexextension@lua{\string tex}
\def\gnuplottexextension@tikz{\string tex}

%
% gnuplot variables getter and setter
%

\def\gpsetvar#1#2{%
  \expandafter\xdef\csname gp@var@#1\endcsname{#2}
}

\def\gpgetvar#1{%
  \csname gp@var@#1\endcsname %
}

%
% some wrapper code
%

% short for a filled path
\def\gpfill#1{\path[line width=0.1\gpbaselw,draw,fill,#1]}

% short for changing the line width
\def\gpsetlinewidth#1{\pgfsetlinewidth{#1\gpbaselw}}

% short for changing the line type
\def\gpsetlinetype#1{\tikzset{gp path/.style={#1,#1 add}}}

% short for changing the dash pattern
\def\gpsetdashtype#1{\tikzset{gp path/.append style={#1}}}

% short for changing the point size
\def\gpsetpointsize#1{\tikzset{gp point/.style={mark size=#1\gpbasems}}}

% wrapper for color settings
\def\gpcolor#1{\tikzset{global #1}}
\tikzset{rgb color/.code={\pgfutil@definecolor{.}{rgb}{#1}\tikzset{color=.}}}
\tikzset{global rgb color/.code={\pgfutil@definecolor{.}{rgb}{#1}\pgfutil@color{.}}}
\tikzset{global color/.code={\pgfutil@color{#1}}}

% prevent plot mark distortions due to changes in the PGF transformation matrix
% use `\gpscalepointstrue' and `\gpscalepointsfalse' for enabling and disabling
% point scaling
% 3-parameter variant gp3point passes style options as well as point type and coordinates
%
\newif\ifgpscalepoints
\tikzset{gp shift only/.style={%
  \ifgpscalepoints\else shift only\fi%
}}
\def\gppoint#1#2{%
  \path[solid] plot[only marks,gp point,mark options={gp shift only},#1] coordinates {#2};%
}
\def\gp3point#1#2#3{%
  \path[solid#2] plot[only marks,gp point,mark options={gp shift only},#1] coordinates {#3};%
}


%
% char size calculation, that might be used with gnuplottex
%
% Example code (needs gnuplottex.sty):
%
%    % calculate the char size when the "gnuplot" style is used
%    \tikzset{gnuplot/.append style={execute at begin picture=\gpcalccharsize}}
%
%    \tikzset{gnuplot/.append style={font=\ttfamily\footnotesize}}
%
%    \begin{tikzpicture}[gnuplot]
%      \begin{gnuplot}[terminal=lua,%
%          terminaloptions={tikz solid nopic charsize \the\gphcharsize,\the\gpvcharsize}]
%        test
%      \end{gnuplot}
%    \end{tikzpicture}
%
%%%
% The `\gpcalccharsize' command fills the lengths \gpvcharsize and \gphcharsize with
% the values of the current default font used within nodes and is meant to be called
% within a tikzpicture environment.
% 
\newdimen\gpvcharsize
\newdimen\gphcharsize
\def\gpcalccharsize{%
  \pgfinterruptboundingbox%
  \pgfsys@begininvisible%
  \node at (0,0) {%
    \global\gphcharsize=1.05\fontcharwd\font`0%
    \global\gpvcharsize=1.05\fontcharht\font`0%
    \global\advance\gpvcharsize by 1.05\fontchardp\font`g%
  };%
  \pgfsys@endinvisible%
  \endpgfinterruptboundingbox%
}

%
%  define a rectangular node in tikz e.g. for the plot area
%
%  #1 node name
%  #2 coordinate of "south west"
%  #3 coordinate of "north east"
%
\def\gpdefrectangularnode#1#2#3{%
  \expandafter\gdef\csname pgf@sh@ns@#1\endcsname{rectangle}%
  \expandafter\gdef\csname pgf@sh@np@#1\endcsname{%
    \def\southwest{#2}%
    \def\northeast{#3}%
  }%
  \pgfgettransform\pgf@temp%
  % once it is defined, no more transformations will be applied, I hope
  \expandafter\xdef\csname pgf@sh@nt@#1\endcsname{\pgf@temp}%
  \expandafter\xdef\csname pgf@sh@pi@#1\endcsname{\pgfpictureid}%
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%  You may want to adapt the following to fit your needs (in your 
%%  individual style file and/or within your document).
%%

%
% style for every plot
%
\tikzset{gnuplot/.style={%
  >=stealth',%
  line cap=round,%
  line join=round,%
}}

\tikzset{gp node left/.style={anchor=mid west,yshift=-.12ex,line width=0pt}}
\tikzset{gp node center/.style={anchor=mid,yshift=-.12ex,line width=0pt}}
\tikzset{gp node right/.style={anchor=mid east,yshift=-.12ex,line width=0pt}}

% basic plot mark size (points)
\newdimen\gpbasems
\gpbasems=.4pt

% basic linewidth
\newdimen\gpbaselw
\gpbaselw=.4pt

% this is the default color for pattern backgrounds
\colorlet{gpbgfillcolor}{white}

% set background color and fill color
\def\gpsetbgcolor#1{%
  \pgfutil@definecolor{gpbgfillcolor}{rgb}{#1}%
  \tikzset{tight background,background rectangle/.style={fill=gpbgfillcolor},show background rectangle}%
}

% this should reverse the normal text node presets, for the
% later referencing as described below
\tikzset{gp refnode/.style={coordinate,yshift=.12ex}}

% to add an empty label with the referenceable name "my node"
% to the plot, just add the following line to your gnuplot
% file:
%
% set label "" at 1,1 font ",gp refnode,name=my node"
%

% enlargement of the bounding box in standalone mode (only used by LaTeX/ConTeXt)
\def\gpbboxborder{0mm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%  The following TikZ-styles are derived from the 'pgf.styles.*' tables
%%  in the Lua script.
%%  To change the number of used styles you should change them there and
%%  regenerate this style file.
%%

% arrow styles settings
\tikzset{gp arrow 1/.style={>=latex}}
\tikzset{gp arrow 2/.style={>=angle 90}}
\tikzset{gp arrow 3/.style={>=angle 60}}
\tikzset{gp arrow 4/.style={>=angle 45}}
\tikzset{gp arrow 5/.style={>=o}}
\tikzset{gp arrow 6/.style={>=*}}
\tikzset{gp arrow 7/.style={>=diamond}}
\tikzset{gp arrow 8/.style={>=open diamond}}
\tikzset{gp arrow 9/.style={>={]}}}
\tikzset{gp arrow 10/.style={>={[}}}
\tikzset{gp arrow 11/.style={>=)}}
\tikzset{gp arrow 12/.style={>=(}}

% plotmark settings
\tikzset{gp mark 0/.style={mark size=.5\pgflinewidth,mark=*}}
\tikzset{gp mark 1/.style={mark=+}}
\tikzset{gp mark 2/.style={mark=x}}
\tikzset{gp mark 3/.style={mark=star}}
\tikzset{gp mark 4/.style={mark=square}}
\tikzset{gp mark 5/.style={mark=square*}}
\tikzset{gp mark 6/.style={mark=o}}
\tikzset{gp mark 7/.style={mark=*}}
\tikzset{gp mark 8/.style={mark=triangle}}
\tikzset{gp mark 9/.style={mark=triangle*}}
\tikzset{gp mark 10/.style={mark=triangle,every mark/.append style={rotate=180}}}
\tikzset{gp mark 11/.style={mark=triangle*,every mark/.append style={rotate=180}}}
\tikzset{gp mark 12/.style={mark=diamond}}
\tikzset{gp mark 13/.style={mark=diamond*}}
\tikzset{gp mark 14/.style={mark=otimes}}
\tikzset{gp mark 15/.style={mark=oplus}}

% pattern settings
\tikzset{gp pattern 0/.style={white}}
\tikzset{gp pattern 1/.style={pattern=north east lines}}
\tikzset{gp pattern 2/.style={pattern=north west lines}}
\tikzset{gp pattern 3/.style={pattern=crosshatch}}
\tikzset{gp pattern 4/.style={pattern=grid}}
\tikzset{gp pattern 5/.style={pattern=vertical lines}}
\tikzset{gp pattern 6/.style={pattern=horizontal lines}}
\tikzset{gp pattern 7/.style={pattern=dots}}
\tikzset{gp pattern 8/.style={pattern=crosshatch dots}}
\tikzset{gp pattern 9/.style={pattern=fivepointed stars}}
\tikzset{gp pattern 10/.style={pattern=sixpointed stars}}
\tikzset{gp pattern 11/.style={pattern=bricks}}

% if the 'tikzplot' option is used the corresponding lines will be smoothed by default
\tikzset{gp plot axes/.style=}
\tikzset{gp plot border/.style=}
\tikzset{gp plot 0/.style=smooth}
\tikzset{gp plot 1/.style=smooth}
\tikzset{gp plot 2/.style=smooth}
\tikzset{gp plot 3/.style=smooth}
\tikzset{gp plot 4/.style=smooth}
\tikzset{gp plot 5/.style=smooth}
\tikzset{gp plot 6/.style=smooth}
\tikzset{gp plot 7/.style=smooth}

% linestyle settings
\tikzset{gp lt axes/.style=dotted}
\tikzset{gp lt border/.style=solid}

% linestyle "addon" settings for overwriting a default linestyle within the
% TeX document via eg. \tikzset{gp lt plot 1 add/.style={fill=black,draw=none}} etc.
\tikzset{gp lt axes add/.style={}}
\tikzset{gp lt border add/.style={}}
\tikzset{gp lt plot 0 add/.style={}}
\tikzset{gp lt plot 1 add/.style={}}
\tikzset{gp lt plot 2 add/.style={}}
\tikzset{gp lt plot 3 add/.style={}}
\tikzset{gp lt plot 4 add/.style={}}
\tikzset{gp lt plot 5 add/.style={}}
\tikzset{gp lt plot 6 add/.style={}}
\tikzset{gp lt plot 7 add/.style={}}
\tikzset{gp lt plot 0/.style={}}
\tikzset{gp lt plot 1/.style={}}
\tikzset{gp lt plot 2/.style={}}
\tikzset{gp lt plot 3/.style={}}
\tikzset{gp lt plot 4/.style={}}
\tikzset{gp lt plot 5/.style={}}
\tikzset{gp lt plot 6/.style={}}
\tikzset{gp lt plot 7/.style={}}

% linestyle color settings
\colorlet{gp lt color axes}{black!30}
\colorlet{gp lt color border}{black}

% dash type settings
% Define this as a macro so that the dash patterns expand later with the current \pgflinewidth.
\def\gpdashlength{\pgflinewidth}
\tikzset{gp dt 0/.style={solid}}
\tikzset{gp dt 1/.style={solid}}
\tikzset{gp dt 2/.style={dash pattern=on 7.5*\gpdashlength off 7.5*\gpdashlength}}
\tikzset{gp dt 3/.style={dash pattern=on 3.75*\gpdashlength off 5.625*\gpdashlength}}
\tikzset{gp dt 4/.style={dash pattern=on 1*\gpdashlength off 2.8125*\gpdashlength}}
\tikzset{gp dt 5/.style={dash pattern=on 11.25*\gpdashlength off 3.75*\gpdashlength on 1*\gpdashlength off 3.75*\gpdashlength}}
\tikzset{gp dt 6/.style={dash pattern=on 5.625*\gpdashlength off 5.625*\gpdashlength on 1*\gpdashlength off 5.625*\gpdashlength}}
\tikzset{gp dt 7/.style={dash pattern=on 3.75*\gpdashlength off 3.75*\gpdashlength on 3.75*\gpdashlength off 11.25*\gpdashlength}}
\tikzset{gp dt 8/.style={dash pattern=on 1*\gpdashlength off 3.75*\gpdashlength on 11.25*\gpdashlength off 3.75*\gpdashlength on 1*\gpdashlength off 3.75*\gpdashlength}}
\tikzset{gp dt solid/.style={solid}}
\tikzset{gp dt axes/.style={dotted}}

% command for switching to colored lines
\def\gpcoloredlines{%
  \colorlet{gp lt color 0}{red}%
  \colorlet{gp lt color 1}{green}%
  \colorlet{gp lt color 2}{blue}%
  \colorlet{gp lt color 3}{magenta}%
  \colorlet{gp lt color 4}{cyan}%
  \colorlet{gp lt color 5}{yellow}%
  \colorlet{gp lt color 6}{orange}%
  \colorlet{gp lt color 7}{purple}%
}

% command for switching to monochrome (black) lines
\def\gpmonochromelines{%
  \colorlet{gp lt color 0}{black}%
  \colorlet{gp lt color 1}{black}%
  \colorlet{gp lt color 2}{black}%
  \colorlet{gp lt color 3}{black}%
  \colorlet{gp lt color 4}{black}%
  \colorlet{gp lt color 5}{black}%
  \colorlet{gp lt color 6}{black}%
  \colorlet{gp lt color 7}{black}%
}

%
% some initialisations
%
% by default all lines will be colored
\gpcoloredlines
\gpsetpointsize{4}
\gpsetlinetype{gp lt solid}
\gpscalepointsfalse
\endinput


==> plots_and_tables/comparison_1.tex <==
\begin{figure*}[ht!]
    \centering
    \small
    %\captionsetup[subfigure]{aboveskip=-1.0\baselineskip}
    \begin{subfigure}[t]{0.5\textwidth}
        \centering
        \begin{gnuplot}[terminal=tikz, terminaloptions={color size 8.0cm,5.5cm fontscale 0.8}]
            load "./gnuplot/common.gp"
    
            KL_file_path = "./data/comparison_100k_samples/KL16g_100k.csv"
            KSG_file_path = "./data/comparison_100k_samples/KSG16g_100k.csv"
            NF_file_path = "./data/comparison_100k_samples/NF16g_100k.csv"
            MINE_file_path = "./data/comparison_100k_samples/MINE16g_100k.csv"
            InfoNCE_file_path = "./data/comparison_100k_samples/InfoNCE16g_100k.csv"
            NWJ_file_path = "./data/comparison_100k_samples/NWJ16g_100k.csv"
            Nishiyama_file_path = "./data/comparison/Nishiyama16g.csv"
            minde_с_file_path = "./data/comparison_100k_samples/minde_res_csv/MINDE_c_16gaussian_100k.csv"
            minde_j_file_path = "./data/comparison_100k_samples/minde_res_csv/MINDE_j_16gaussian_100k.csv"
            bridge_file_path = "./data/comparison_100k_samples/bridge16g_100k.csv"
            
            confidence = 0.99
            max_y = 10.0
    
            load "./gnuplot/estmi_mi_1.gp"
        \end{gnuplot}
        \caption{$16\times 16$ images (Gaussians)}
    \end{subfigure}%
    \begin{subfigure}[t]{0.5\textwidth}
        \centering
        \begin{gnuplot}[terminal=tikz, terminaloptions={color size 8.0cm,5.5cm fontscale 0.8}]
            load "./gnuplot/common.gp"

            KL_file_path = "./data/comparison_100k_samples/KL32g_100k.csv"
            KSG_file_path = "./data/comparison_100k_samples/KSG32g_100k.csv"
            NF_file_path = "./data/comparison_100k_samples/NF32g_100k.csv"
            MINE_file_path = "./data/comparison_100k_samples/MINE32g_100k.csv"
            InfoNCE_file_path = "./data/comparison_100k_samples/InfoNCE32g_100k.csv"
            NWJ_file_path = "./data/comparison_100k_samples/NWJ32g_100k.csv"
            Nishiyama_file_path = "./data/comparison/Nishiyama32g.csv"
            minde_с_file_path = "./data/comparison_100k_samples/minde_res_csv/MINDE_c_32gaussian_100k.csv"
            minde_j_file_path = "./data/comparison_100k_samples/minde_res_csv/MINDE_j_32gaussian_100k.csv"
            bridge_file_path = "./data/comparison_100k_samples/bridge32g_100k.csv"
            
            confidence = 0.99
            max_y = 10.0
    
            load "./gnuplot/estmi_mi_1.gp"
        \end{gnuplot}
        \caption{$32\times 32$ images (Gaussians)}
    \end{subfigure}

    \begin{subfigure}[t]{0.5\textwidth}
        \centering
        \begin{gnuplot}[terminal=tikz, terminaloptions={color size 8.0cm,5.5cm fontscale 0.8}]
            load "./gnuplot/common.gp"
    
            KL_file_path = "./data/comparison_100k_samples/KL16r_100k.csv"
            KSG_file_path = "./data/comparison_100k_samples/KSG16r_10k.csv"
            NF_file_path = "./data/comparison_100k_samples/NF16r_100k.csv"
            MINE_file_path = "./data/comparison_100k_samples/MINE16r_100k.csv"
            InfoNCE_file_path = "./data/comparison_100k_samples/InfoNCE16r_100k.csv"
            NWJ_file_path = "./data/comparison_100k_samples/NWJ16r_100k.csv"
            Nishiyama_file_path = "./data/comparison/Nishiyama16r.csv"
            minde_с_file_path = "./data/comparison_100k_samples/minde_res_csv/MINDE_c_16rectangle_100k.csv"
            minde_j_file_path = "./data/comparison_100k_samples/minde_res_csv/MINDE_j_16rectangle_100k.csv"
            bridge_file_path = "./data/comparison_100k_samples/bridge16r_100k.csv"
            
            confidence = 0.99
            max_y = 10.0
    
            load "./gnuplot/estmi_mi_1.gp"
        \end{gnuplot}
        \caption{$16\times 16$ images (Rectangles)}
    \end{subfigure}%
    \begin{subfigure}[t]{0.5\textwidth}
        \centering
        \begin{gnuplot}[terminal=tikz, terminaloptions={color size 8.0cm,5.5cm fontscale 0.8}]
            load "./gnuplot/common.gp"
    
    
            KL_file_path = "./data/comparison_100k_samples/KL32r_100k.csv"
            NF_file_path = "./data/comparison_100k_samples/NF32r_100k.csv"
            MINE_file_path = "./data/comparison_100k_samples/MINE32r_100k.csv"
            Nishiyama_file_path = "./data/comparison/Nishiyama32r.csv"
            minde_с_file_path = "./data/comparison_100k_samples/minde_res_csv/MINDE_c_32rectangle_100k.csv"
            minde_j_file_path = "./data/comparison_100k_samples/minde_res_csv/MINDE_j_32rectangle_100k.csv"
            bridge_file_path = "./data/comparison_100k_samples/bridge32r_100k.csv"
            
            confidence = 0.99
            max_y = 10.0
            key_pos="lower"
    
            load "./gnuplot/estmi_mi_1.gp"
        \end{gnuplot}
        \caption{$32\times 32$ images (Rectangles)}
    \end{subfigure}
    %
    \caption{Comparison of the selected estimators. Along $ x $ axes is $ I(X_0;X_1) $, along $ y $ axes is MI estimate $ \hat I(X_0;X_1) $. We plot 99\% asymptotic CIs acquired from different seed runs. Number of seeds for \ourestname{} and $\normal$-MIENF is 3 and 5 for all the other methods. $100$k samples were used for neural methods training and $10$k for validation.}
    \label{figure:compare_methods_images_1}
    %\vskip 0.2in
\end{figure*}

==> plots_and_tables/comparison_2.tex <==
\begin{figure*}[ht!]
    \centering
    \small
    % \captionsetup[subfigure]{aboveskip=-1.0\baselineskip}
    % \begin{subfigure}[t]{0.5\textwidth}
    %     \centering
    %     \begin{gnuplot}[terminal=tikz, terminaloptions={color size 8.0cm,5.5cm fontscale 0.8}]
    %         load "./gnuplot/common.gp"
    
    %         MINE_file_path = "./data/comparison_100k_samples/MINE16g_100k.csv"
    %         Nishiyama_file_path = "./data/comparison/Nishiyama16g.csv"
    %         minde_с_file_path = "./data/comparison_100k_samples/minde_res_csv/MINDE_c_16gaussian_100k.csv"
    %         minde_j_file_path = "./data/comparison_100k_samples/minde_res_csv/MINDE_j_16gaussian_100k.csv"
    %         bridge_file_path = "./data/comparison_100k_samples/bridge16g_100k.csv"
            
    %         confidence = 0.99
    %         max_y = 10.0
    
    %         load "./gnuplot/estmi_mi_2.gp"
    %     \end{gnuplot}
    %     \caption{$16\times 16$ images (Gaussians)}
    % \end{subfigure}%
    \begin{subfigure}[t]{0.45\textwidth}
        \centering
        \begin{gnuplot}[terminal=tikz, terminaloptions={color size 8.0cm,5.5cm fontscale 0.8}]
            load "./gnuplot/common.gp"

            MINE_file_path = "./data/comparison_100k_samples/MINE32g_100k.csv"
            Nishiyama_file_path = "./data/comparison/Nishiyama32g.csv"
            minde_с_file_path = "./data/comparison_100k_samples/minde_res_csv/MINDE_c_32gaussian_100k.csv"
            minde_j_file_path = "./data/comparison_100k_samples/minde_res_csv/MINDE_j_32gaussian_100k.csv"
            bridge_file_path = "./data/comparison_100k_samples/bridge32g_100k.csv"
            
            confidence = 0.99
            max_y = 10.0
    
            load "./gnuplot/estmi_mi_2.gp"
        \end{gnuplot}
        \caption{$32\times 32$ images (Gaussians)}
    \end{subfigure}
    \begin{subfigure}[t]{0.45\textwidth}
        \centering
        \begin{gnuplot}[terminal=tikz, terminaloptions={color size 8.0cm,5.5cm fontscale 0.8}]
            load "./gnuplot/common.gp"
    
    
            MINE_file_path = "./data/comparison_100k_samples/MINE32r_100k.csv"
            Nishiyama_file_path = "./data/comparison/Nishiyama32r.csv"
            minde_с_file_path = "./data/comparison_100k_samples/minde_res_csv/MINDE_c_32rectangle_100k.csv"
            minde_j_file_path = "./data/comparison_100k_samples/minde_res_csv/MINDE_j_32rectangle_100k.csv"
            bridge_file_path = "./data/comparison_100k_samples/bridge32r_100k.csv"
            
            confidence = 0.99
            max_y = 10.0
            key_pos="lower"
    
            load "./gnuplot/estmi_mi_2.gp"
        \end{gnuplot}
        \caption{$32\times 32$ images (Rectangles)}
    \end{subfigure}
    %
    \caption{Comparison of the selected estimators. Along $ x $ axes is $ I(X_0;X_1) $, along $ y $ axes is MI estimate $ \hat I(X_0;X_1) $. We plot 99\% asymptotic CIs acquired from different seed runs. Number of seeds for \ourestname{} and $\normal$-MIENF is 3 and 5 for all the other methods. $100$k samples were used for neural methods training and $10$k for validation.}
    \label{figure:compare_methods_images_2}
    %\vskip 0.2in
\end{figure*}



==> plots_and_tables/comparison_old.tex <==
\begin{figure*}[t!]
    \vspace{-10mm}
    \centering
    \small
    % \hspace{-15mm}
    %\captionsetup[subfigure]{aboveskip=-1.0\baselineskip}
    \begin{subfigure}[t]{0.5\textwidth}
        \centering
        \hspace{-12mm}
        \begin{gnuplot}[terminal=tikz, terminaloptions={color size 8cm,6cm fontscale 0.6}]
            load "./gnuplot/common.gp"
            
            KL_file_path_d_5 = "./data/WKL_bad/KL16g_100k_d5.csv"
            KL_file_path = "./data/comparison_100k_samples/KL16g_100k.csv"
            KSG_file_path = "./data/comparison_100k_samples/KSG16g_100k.csv"
            NF_file_path = "./data/comparison_100k_samples/NF16g_100k.csv"
            MINE_file_path = "./data/comparison_100k_samples/MINE16g_100k.csv"
            InfoNCE_file_path = "./data/comparison_100k_samples/InfoNCE16g_100k.csv"
            NWJ_file_path = "./data/comparison_100k_samples/NWJ16g_100k.csv"
            Nishiyama_file_path = "./data/comparison/Nishiyama16g.csv"
            bridge_file_path = "./data/comparison_100k_samples/bridge16g_100k.csv"
            minde_с_file_path = "./data/comparison_100k_samples/minde_res_csv/MINDE_c_16gaussian_100k.csv"
            minde_j_file_path = "./data/comparison_100k_samples/minde_res_csv/MINDE_j_16gaussian_100k.csv"
            
            confidence = 0.99
            max_y = 10.0
    
            load "./gnuplot/estmi_mi.gp"
        \end{gnuplot}
        \vspace{-6mm}
        \caption{$16\times 16$ images (Gaussians)}
        \vspace{1mm}
    \end{subfigure}%
    \begin{subfigure}[t]{0.5\textwidth}
        \centering
        \begin{gnuplot}[terminal=tikz, terminaloptions={color size 8cm,6cm fontscale 0.6}]
            load "./gnuplot/common.gp"
    
            KL_file_path_d_5 = "./data/WKL_bad/KL32g_100k_d5.csv"
            KL_file_path = "./data/comparison_100k_samples/KL32g_100k.csv"
            KSG_file_path = "./data/comparison_100k_samples/KSG32g_100k.csv"
            NF_file_path = "./data/comparison_100k_samples/NF32g_100k.csv"
            MINE_file_path = "./data/comparison_100k_samples/MINE32g_100k.csv"
            InfoNCE_file_path = "./data/comparison_100k_samples/InfoNCE32g_100k.csv"
            NWJ_file_path = "./data/comparison_100k_samples/NWJ32g_100k.csv"
            minde_с_file_path = "./data/comparison_100k_samples/minde_res_csv/MINDE_c_32gaussian_100k.csv"
            Nishiyama_file_path = "./data/comparison/Nishiyama32g.csv"
            bridge_file_path = "./data/comparison_100k_samples/bridge32g_100k.csv"
            minde_j_file_path = "./data/comparison_100k_samples/minde_res_csv/MINDE_j_32gaussian_100k.csv"
            
            confidence = 0.99
            max_y = 10.0
    
            load "./gnuplot/estmi_mi.gp"
        \end{gnuplot}
        \vspace{-6mm}
        \caption{$32\times 32$ images (Gaussians)}
        \vspace{1mm}
    \end{subfigure}
    \vspace{-2mm}

    % \vspace{4mm}
    \begin{subfigure}[t]{0.5\textwidth}
        \centering
        \hspace{-12mm}
        \begin{gnuplot}[terminal=tikz, terminaloptions={color size 8cm,6cm fontscale 0.6}]
            load "./gnuplot/common.gp"
    
            KL_file_path_d_5 = "./data/WKL_bad/KL16r_100k_d5.csv"
            KL_file_path = "./data/comparison_100k_samples/KL16r_100k.csv"
            KSG_file_path = "./data/comparison_100k_samples/KSG16r_10k.csv"
            NF_file_path = "./data/comparison_100k_samples/NF16r_100k.csv"
            MINE_file_path = "./data/comparison_100k_samples/MINE16r_100k.csv"
            InfoNCE_file_path = "./data/comparison_100k_samples/InfoNCE16r_100k.csv"
            NWJ_file_path = "./data/comparison_100k_samples/NWJ16r_100k.csv"
            Nishiyama_file_path = "./data/comparison/Nishiyama16r.csv"
            bridge_file_path = "./data/comparison_100k_samples/bridge16r_100k.csv"
            minde_с_file_path = "./data/comparison_100k_samples/minde_res_csv/MINDE_c_16rectangle_100k.csv"
            minde_j_file_path = "./data/comparison_100k_samples/minde_res_csv/MINDE_j_16rectangle_100k.csv"
            
            confidence = 0.99
            max_y = 10.0
    
            load "./gnuplot/estmi_mi.gp"
        \end{gnuplot}
        \vspace{-6mm}
        \caption{$16\times 16$ images (Rectangles)}
        \vspace{1mm}
    \end{subfigure}%
    \begin{subfigure}[t]{0.5\textwidth}
        \centering
        \begin{gnuplot}[terminal=tikz, terminaloptions={color size 8cm,6cm fontscale 0.6}]
            load "./gnuplot/common.gp"
    
            KL_file_path_d_5 = "./data/WKL_bad/KL32r_100k_d5.csv"
            KL_file_path = "./data/comparison_100k_samples/KL32r_100k.csv"
            KSG_file_path = "./data/comparison_100k_samples/KSG32r_10k.csv"
            NF_file_path = "./data/comparison_100k_samples/NF32r_100k.csv"
            MINE_file_path = "./data/comparison_100k_samples/MINE32r_100k.csv"
            InfoNCE_file_path = "./data/comparison_100k_samples/InfoNCE32r_100k.csv"
            NWJ_file_path = "./data/comparison_100k_samples/NWJ32r_100k.csv"
            Nishiyama_file_path = "./data/comparison/Nishiyama32r.csv"
            bridge_file_path = "./data/comparison_100k_samples/bridge32r_100k.csv"
            minde_с_file_path = "./data/comparison_100k_samples/minde_res_csv/MINDE_c_32rectangle_100k.csv"
            minde_j_file_path = "./data/comparison_100k_samples/minde_res_csv/MINDE_j_32rectangle_100k.csv"
            
            confidence = 0.99
            max_y = 10.0
            key_pos="lower"
    
            load "./gnuplot/estmi_mi.gp"
        \end{gnuplot}
        \vspace{-6mm}
        \caption{$32\times 32$ images (Rectangles)}
        \vspace{1mm}
    \end{subfigure}
    \vspace{-2mm}
    %
    \caption{Comparison of the MI estimators. Along $ x $ axes is $ I(X_0;X_1) $, along $ y $ axes is MI estimate $ \hat I(X_0;X_1) $. We plot 99\% confidence intervals acquired from different seed runs. Number of seeds for \ourestname{}, $\normal$-MIENF, MINDE is 3 and 5 for all the other methods. $100$k samples were used for neural methods training and $10$k for validation. \underline{MAE} can be seen at Table~\ref{tab:image_data_results}. AE+WKL 5-NN (ib) and (d=5) stand for the versions with \underline{inductive bias} and latent dimensionality of 5 respectively.}
    \label{figure:compare_methods_images}
    %\vskip 0.2in
    
    \vspace{-5mm}
\end{figure*}

==> plots_and_tables/image_data_examples.tex <==

\begin{figure*}[t!]
    \centering
    \begin{subfigure}[b]{0.5\textwidth}
        \captionsetup{skip=0.5\baselineskip}
        \centering
        \includegraphics[width=0.95\textwidth]{figures/paired_gaussian_32_mi_5_eps_1_predict_vector_field_input_x_5.png}
        \caption{Gaussians data samples} \label{fig:image_samples_a}
    \end{subfigure}%
    %
    \begin{subfigure}[b]{0.5\textwidth}
        \captionsetup{skip=0.5\baselineskip}
        \centering
        \includegraphics[width=0.95\textwidth]{figures/paired_rectangle_32_mi_5_eps_1_predict_vector_field_input_x_5.png}
        \caption{Rectangles data samples}\label{fig:image_samples_b}
    \end{subfigure}
    % \vspace{0.3mm}
    
    
    \caption{ Examples of synthetic images from the \cite{butakov2024normflows} benchmark can be seen at \cref{fig:image_samples_a,fig:image_samples_b}.}
    \label{figure:synthetic_images_examples_1}
    \vspace{-5mm}
\end{figure*}

==> plots_and_tables/low_dim_bench_table_old.tex <==

\begin{table*}[t!]
\vspace*{-7mm}
\caption{Mean MI estimates over $ 10 $ seeds using $ 10 $k test samples against ground truth (GT), adopted from~\cite{franzese2024minde}. Color indicates relative
negative (red) and positive bias (blue). Size of train dataset for every neural method is 100k. All the methods for comparison, except for the NVF and JVF \cite{dahlkeflow}, were taken from \cite{czyz2023beyond_normal,franzese2024minde}. List of abbreviations (\textit{Mn}: Multinormal,  \textit{St}: Student-t, \textit{Nm}: Normal, \textit{Hc}: Half-cube, \textit{Sp}: Spiral). Methods explosion is abbreviated by $\infty$.
}
\label{tab:benchmark}
\renewcommand{\tabcolsep}{0.0pt}
\tiny

\resizebox{\textwidth}{!}{
\begin{tabular}{lcrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrr}
\toprule

GT & Method Type & 0.2 & 0.4 & 0.3 & 0.4 & 0.4 & 0.4 & 0.4 & 1.0 & 1.0 & 1.0 & 1.0 & 0.3 & 1.0 & 1.3 & 1.0 & 0.4 & 1.0 & 0.6 & 1.6 & 0.4 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 &
0.2 & 0.4 &
0.2 & 0.3 & 0.2 & 0.4 & 0.3 & 0.4 & 1.7 & 0.3 & 0.4 \\

\midrule

\textbf{\ourestname (ours)} & Bridge Matching & {\cellcolor[HTML]{DAE1EB}} 0.3 & {\cellcolor[HTML]{DAE1EB}} 0.5 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{D4DDE9}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & 
{\cellcolor[HTML]{E188A2}} 0.0 & {\cellcolor[HTML]{DB6185}} 0.0 & 
{\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{D4DDE9}} 0.5 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{D4DDE9}} 0.5 & {\cellcolor[HTML]{E7ADBE}} 1.3 & {\cellcolor[HTML]{DAE1EB}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\

\midrule

NVF & \multirow{2}{*}{Flow} & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{AFC4DD}} 0.6 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{EED3DB}} 1.5 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED3DB}} 0.8 & {\cellcolor[HTML]{DB6185}} 0.5 & {\cellcolor[HTML]{DB6185}} 0.6 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & 
{\cellcolor[HTML]{DB6185}} $\infty$ & {\cellcolor[HTML]{DB6185}} $\infty$ & 
{\cellcolor[HTML]{DB6185}} $\infty$ & {\cellcolor[HTML]{BCCCE1}} 0.5 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{DB6185}} -0.4 & {\cellcolor[HTML]{D4DDE9}} 0.4 & {\cellcolor[HTML]{E9BAC8}} 0.2 & {\cellcolor[HTML]{E9BAC8}} 1.5 & {\cellcolor[HTML]{E9BAC8}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\

JVF & & {\cellcolor[HTML]{E9BAC8}} 0.0 & {\cellcolor[HTML]{DB6185}} 0.0 & {\cellcolor[HTML]{DB6185}} 0.0 & {\cellcolor[HTML]{DB6185}} 0.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{F2F2F2}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED3DB}} 0.8 & {\cellcolor[HTML]{DB6185}} 0.3 & {\cellcolor[HTML]{DB6185}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{EED3DB}} 0.9 &
{\cellcolor[HTML]{4479BB}} 1.8 & {\cellcolor[HTML]{4479BB}} 2.7 & 
{\cellcolor[HTML]{E188A2}} 0.0 & {\cellcolor[HTML]{E188A2}} 0.1 & {\cellcolor[HTML]{E188A2}} 0.0 & {\cellcolor[HTML]{DB6185}} 0.1 & {\cellcolor[HTML]{DB6185}} 0.0 & {\cellcolor[HTML]{D4DDE9}} 0.0 & {\cellcolor[HTML]{E9BAC8}} 1.6 & {\cellcolor[HTML]{DAE1EB}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\

\midrule

MINDE--\textsc{j} ($\sigma=1$) \ & \multirow{4}{*}{Diffusion} & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{D4DDE9}} 1.1 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{EED3DB}} 1.2 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{D4DDE9}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & 
{\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & 
{\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{D4DDE9}} 0.5 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{D4DDE9}} 0.5 & {\cellcolor[HTML]{EED3DB}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\


MINDE--\textsc{j} &  &  {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{AFC4DD}} 1.2 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{D4DDE9}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{D4DDE9}} 1.1 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{D4DDE9}} 1.1 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & 
{\cellcolor[HTML]{EED3DB}} 0.1 & {\cellcolor[HTML]{E7ADBE}} 0.2 & 
{\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{D4DDE9}} 0.5 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\



MINDE--\textsc{c} ($\sigma=1$) & & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{F2F2F2}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.9 & 
{\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{EED9DF}} 0.3 & 
{\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\



MINDE--\textsc{c} &  & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{F2F2F2}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{EED9DF}} 0.1 & 
{\cellcolor[HTML]{EED9DF}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.2 & 
{\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\

\midrule
MINE & \multirow{7}{*}{Classical} & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED3DB}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{F2F2F2}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{E7ADBE}} 0.8 & {\cellcolor[HTML]{E188A2}} 0.7 & {\cellcolor[HTML]{DB6185}} 0.6 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{E7ADBE}} 0.0 & 
{\cellcolor[HTML]{DB6185}} 0.0 & {\cellcolor[HTML]{EED3DB}} 0.1 & 
{\cellcolor[HTML]{E7ADBE}} 0.1 & {\cellcolor[HTML]{EED3DB}} 0.1 & {\cellcolor[HTML]{E7ADBE}} 0.2 & {\cellcolor[HTML]{EED3DB}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
InfoNCE & & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{F2F2F2}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{E7ADBE}} 0.8 & {\cellcolor[HTML]{E7ADBE}} 0.8 & {\cellcolor[HTML]{E7ADBE}} 0.8 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.2 & 
{\cellcolor[HTML]{EED3DB}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.2 & 
{\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
D-V & & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{F2F2F2}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{E7ADBE}} 0.8 & {\cellcolor[HTML]{E7ADBE}} 0.8 & {\cellcolor[HTML]{E7ADBE}} 0.8 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{E7ADBE}} 0.0 & 
{\cellcolor[HTML]{DB6185}} 0.0 & {\cellcolor[HTML]{EED3DB}} 0.1 & 
{\cellcolor[HTML]{E7ADBE}} 0.1 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{E7ADBE}} 0.2 & {\cellcolor[HTML]{EED3DB}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\
NWJ & & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.3 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{F2F2F2}} 1.6 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{E7ADBE}} 0.8 & {\cellcolor[HTML]{E7ADBE}} 0.8 & {\cellcolor[HTML]{E7ADBE}} 0.8 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{E7ADBE}} 0.0 & 
{\cellcolor[HTML]{DB6185}} 0.0 & {\cellcolor[HTML]{E7ADBE}} 0.0 & 
{\cellcolor[HTML]{D53D69}} -0.6 & {\cellcolor[HTML]{EED3DB}} 0.1 & {\cellcolor[HTML]{E188A2}} 0.1 & {\cellcolor[HTML]{EED3DB}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\



DoE (Gaussian) & & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{DAE1EB}} 0.5 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{BCCCE1}} 0.6 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{DAE1EB}} 0.4 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{4479BB}} 7.8 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{BCCCE1}} 0.6 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{4479BB}} 1.3 &  & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{DA5C81}} 0.5 & {\cellcolor[HTML]{DF7B98}} 0.6 & {\cellcolor[HTML]{DF7B98}} 0.6 & {\cellcolor[HTML]{DF7B98}} 0.6 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{E9BAC8}} 0.8 & 
{\cellcolor[HTML]{4479BB}} 6.7 & {\cellcolor[HTML]{4479BB}} 7.9 & 
{\cellcolor[HTML]{4479BB}} 1.8 & {\cellcolor[HTML]{4479BB}} 2.5 & {\cellcolor[HTML]{7FA2CE}} 0.6 & {\cellcolor[HTML]{4479BB}} 4.2 & {\cellcolor[HTML]{4479BB}} 1.2 & {\cellcolor[HTML]{EED9DF}} 1.6 & {\cellcolor[HTML]{E9BAC8}} 0.1 & {\cellcolor[HTML]{F2F2F2}} 0.4 &  \\
DoE (Logistic) & & {\cellcolor[HTML]{EED9DF}} 0.1 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED9DF}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{DF7B98}} 0.6 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{4479BB}} 7.8 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{BCCCE1}} 0.6 & {\cellcolor[HTML]{EED9DF}} 0.9 & {\cellcolor[HTML]{4479BB}} 1.3 &  & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{DAE1EB}} 1.1 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{DA5C81}} 0.5 & {\cellcolor[HTML]{DF7B98}} 0.6 & {\cellcolor[HTML]{DF7B98}} 0.6 & {\cellcolor[HTML]{E49AAF}} 0.7 & {\cellcolor[HTML]{E9BAC8}} 0.8 & {\cellcolor[HTML]{E9BAC8}} 0.8 & 
% & {\cellcolor[HTML]{4479BB}} 2.0 &
{\cellcolor[HTML]{9DB7D7}} 0.5 & {\cellcolor[HTML]{628DC4}} 0.8 & {\cellcolor[HTML]{DAE1EB}} 0.3 & {\cellcolor[HTML]{4479BB}} 1.5 & {\cellcolor[HTML]{9DB7D7}} 0.6 & {\cellcolor[HTML]{EED9DF}} 1.6 & {\cellcolor[HTML]{E9BAC8}} 0.1 & {\cellcolor[HTML]{F2F2F2}} 0.4 & \\

KSG & & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{EED3DB}} 0.2 & {\cellcolor[HTML]{E7ADBE}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{D53D69}} 0.2 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{E188A2}} 0.7 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{D53D69}} 0.2 & {\cellcolor[HTML]{E7ADBE}} 1.1 & {\cellcolor[HTML]{F2F2F2}} 1.0 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{E188A2}} 0.7 & {\cellcolor[HTML]{F2F2F2}} 0.6 & {\cellcolor[HTML]{E188A2}} 1.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{D53D69}} 0.2 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{E188A2}} 0.7 & {\cellcolor[HTML]{D53D69}} 0.2 & {\cellcolor[HTML]{E188A2}} 0.7 & {\cellcolor[HTML]{DB6185}} 0.6 & {\cellcolor[HTML]{D53D69}} 0.2 & {\cellcolor[HTML]{EED3DB}} 0.9 & {\cellcolor[HTML]{E188A2}} 0.7 & {\cellcolor[HTML]{F2F2F2}} 0.2 & {\cellcolor[HTML]{E7ADBE}} 0.2 & {\cellcolor[HTML]{EED3DB}} 0.1 & {\cellcolor[HTML]{E7ADBE}} 0.1 & {\cellcolor[HTML]{EED3DB}} 0.1 & {\cellcolor[HTML]{E7ADBE}} 0.2 & {\cellcolor[HTML]{EED3DB}} 0.2 & {\cellcolor[HTML]{F2F2F2}} 0.4 & {\cellcolor[HTML]{F2F2F2}} 1.7 & {\cellcolor[HTML]{F2F2F2}} 0.3 & {\cellcolor[HTML]{F2F2F2}} 0.4 \\


\midrule
 & & \begin{sideways} Asinh @ \textit{St} 1 × 1 (dof=1)\end{sideways} & 
\begin{sideways}Asinh @ \textit{St} 2 × 2 (dof=1) \end{sideways}& 
\begin{sideways}Asinh @ \textit{St} 3 × 3 (dof=2) \end{sideways}& 
\begin{sideways}Asinh @ \textit{St} 5 × 5 (dof=2)\end{sideways} &
\begin{sideways} Bimodal 1 × 1 \end{sideways}&
\begin{sideways}Bivariate \textit{Nm} 1 × 1\end{sideways} &
\begin{sideways} \textit{Hc} @ Bivariate \textit{Nm} 1 × 1\end{sideways} &
\begin{sideways} \textit{Hc} @ \textit{Mn} 25 × 25 (2-pair)\end{sideways} &
\begin{sideways} \textit{Hc} @ \textit{Mn} 3 × 3 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Hc} @ \textit{Mn} 5 × 5 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Mn} 2 × 2 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Mn} 2 × 2 (dense)\end{sideways} &
\begin{sideways} \textit{Mn} 25 × 25 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Mn} 25 × 25 (dense) \end{sideways}& 
\begin{sideways} \textit{Mn} 3 × 3 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Mn} 3 × 3 (dense) \end{sideways}&
\begin{sideways} \textit{Mn} 5 × 5 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Mn} 5 × 5 (dense) \end{sideways}&
\begin{sideways} \textit{Mn} 50 × 50 (dense) \end{sideways}& 
\begin{sideways} \textit{Nm} CDF @ Bivariate \textit{Nm} 1 × 1\end{sideways} &
\begin{sideways} \textit{Nm} CDF @ \textit{Mn} 25 × 25 (2-pair) \end{sideways}&
\begin{sideways} \textit{Nm} CDF @ \textit{Mn} 3 × 3 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Nm} CDF @ \textit{Mn} 5 × 5 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Sp} @ \textit{Mn} 25 × 25 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Sp} @ \textit{Mn} 3 × 3 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Sp} @ \textit{Mn} 5 × 5 (2-pair)\end{sideways} & 
\begin{sideways} \textit{Sp} @ \textit{Nm} CDF @ \textit{Mn} 25 × 25 (2-pair) \end{sideways}&
\begin{sideways} \textit{Sp} @ \textit{Nm} CDF @ \textit{Mn} 3 × 3 (2-pair) \end{sideways}& 
\begin{sideways} \textit{Sp} @ \textit{Nm} CDF @ \textit{Mn} 5 × 5 (2-pair) \end{sideways}&
\begin{sideways} \textit{St} 1 × 1 (dof=1)\end{sideways} & 
\begin{sideways} \textit{St} 2 × 2 (dof=1)\end{sideways} &
\begin{sideways} \textit{St} 2 × 2 (dof=2) \end{sideways}& 
\begin{sideways} \textit{St} 3 × 3 (dof=2)\end{sideways} & 
\begin{sideways} \textit{St} 3 × 3 (dof=3)\end{sideways} & 
\begin{sideways} \textit{St} 5 × 5 (dof=2)\end{sideways} & 
\begin{sideways} \textit{St} 5 × 5 (dof=3) \end{sideways}& 
\begin{sideways} Swiss roll 2 × 1 \end{sideways}&
\begin{sideways} Uniform 1 × 1 (additive noise=0.1) \end{sideways}&
\begin{sideways} Uniform 1 × 1 (additive noise=0.75) \end{sideways}& 
\begin{sideways} Wiggly @ Bivariate \textit{Nm} 1 × 1 \end{sideways} \\

\bottomrule
\end{tabular}}

% \vspace{-2mm}

\end{table*}


==> plots_and_tables/wkl_bad_old.tex <==

\begin{figure*}[ht!]
    \centering
    \small
    \begin{subfigure}[t]{0.5\textwidth}
        \centering
        \begin{gnuplot}[terminal=tikz, terminaloptions={color size 7.5cm,4.2cm fontscale 0.8}]
            load "./gnuplot/common.gp"
    
            KSG_file_path = "./data/comparison_100k_samples/KSG16g_100k.csv"
            NF_file_path = "./data/comparison_100k_samples/NF16g_100k.csv"
            MINE_file_path = "./data/comparison_100k_samples/MINE16g_100k.csv"
            InfoNCE_file_path = "./data/comparison_100k_samples/InfoNCE16g_100k.csv"
            NWJ_file_path = "./data/comparison_100k_samples/NWJ16g_100k.csv"
            Nishiyama_file_path = "./data/comparison/Nishiyama16g.csv"
            bridge_file_path = "./data/comparison_100k_samples/bridge16g_100k.csv"
            minde_с_file_path = "./data/comparison_100k_samples/minde_res_csv/MINDE_c_16gaussian_100k.csv"
            minde_j_file_path = "./data/comparison_100k_samples/minde_res_csv/MINDE_j_16gaussian_100k.csv"
            KL_2_file_path = "./data/comparison_100k_samples/KL16g_100k.csv"
            KL_4_file_path = "./data/WKL_bad/KL16g_100k_d4.csv"
            KL_5_file_path = "./data/WKL_bad/KL16g_100k_d5.csv"
            
            confidence = 0.99
            #max_y = 10.0
    
            load "./gnuplot/estmi_wkl_full_plot.gp"
        \end{gnuplot}
        \caption{$16\times 16$ images (Gaussians)}
    \end{subfigure}%
    \begin{subfigure}[t]{0.5\textwidth}
        \centering
        \begin{gnuplot}[terminal=tikz, terminaloptions={color size 7.5cm,4.2cm fontscale 0.8}]
            load "./gnuplot/common.gp"
    
            #KL_file_path = "./data/WKL_bad/KL32g_100k_bad.csv"
            
            KSG_file_path = "./data/comparison_100k_samples/KSG32g_100k.csv"
            NF_file_path = "./data/comparison_100k_samples/NF32g_100k.csv"
            MINE_file_path = "./data/comparison_100k_samples/MINE32g_100k.csv"
            InfoNCE_file_path = "./data/comparison_100k_samples/InfoNCE32g_100k.csv"
            minde_с_file_path = "./data/comparison_100k_samples/minde_res_csv/MINDE_c_32gaussian_100k.csv"
            Nishiyama_file_path = "./data/comparison/Nishiyama32g.csv"
            NWJ_file_path = "./data/comparison_100k_samples/NWJ32g_100k.csv"
            bridge_file_path = "./data/comparison_100k_samples/bridge32g_100k.csv"
            minde_j_file_path = "./data/comparison_100k_samples/minde_res_csv/MINDE_j_32gaussian_100k.csv"
            KL_2_file_path = "./data/comparison_100k_samples/KL32g_100k.csv"
            KL_4_file_path = "./data/WKL_bad/KL32g_100k_d4.csv"
            KL_5_file_path = "./data/WKL_bad/KL32g_100k_d5.csv"
            
            confidence = 0.99
            #max_y = 10.0
    
            load "./gnuplot/estmi_wkl_full_plot.gp"
        \end{gnuplot}
        \caption{$32\times 32$ images (Gaussians)}
    \end{subfigure}
    \caption{Results for AE+WKL $5$-NN for different bottleneck dimensionality. Along $ x $ axes is $ I(X_0;X_1) $, along $ y $ axes is MI estimate $ \hat I(X_0;X_1) $. We plot 99\% asymptotic CIs acquired from different seed runs ($ 5 $ seeds in total).}
    \label{figure:compare_methods_images_WKL_bad}
    %\vskip 0.2in
\end{figure*}


